Spreads and Packings of PG(3,2), Formally!

We study how to formalize in the Coq proof assistant the smallest projective space PG(3,2). We then describe formally the spreads and packings of PG(3,2), as well as some of their properties. The formalization is rather straightforward, however as the number of objects at stake increases rapidly, we need to exploit some symmetry arguments as well as smart proof techniques to make proof search and verification faster and thus tractable using the Coq proof assistant. This work can be viewed as a first step towards formalizing projective spaces of higher dimension, e.g. PG(4,2), or larger order, e.g. PG(3,3).

==> eptcsdata.tex <==
\providecommand{\firstpage}{107}
\providecommand{\publicationstatus}{Jani\v{c}i\'c, Kov\'acs (Eds.): Automated Deduction in Geometry (ADG 2021)\\
EPTCS 352, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.352.12}{10.4204/EPTCS.352.12}}
\pdfoutput=1

